BnTTS: Few-Shot Speaker Adaptation in Low-Resource Setting

This paper introduces BnTTS (Bangla Text-To-Speech), the first framework for Bangla speaker adaptation-based TTS, designed to bridge the gap in Bangla speech synthesis using minimal training data. Building upon the XTTS architecture, our approach integrates Bangla into a multilingual TTS pipeline, with modifications to account for the phonetic and linguistic characteristics of the language. We pre-train BnTTS on 3.85k hours of Bangla speech dataset with corresponding text labels and evaluate performance in both zero-shot and few-shot settings on our proposed test dataset. Empirical evaluations in few-shot settings show that BnTTS significantly improves the naturalness, intelligibility, and speaker fidelity of synthesized Bangla speech. Compared to state-of-the-art Bangla TTS systems, BnTTS exhibits superior performance in Subjective Mean Opinion Score (SMOS), Naturalness, and Clarity metrics.

==> sections/BnTTS.tex <==
% \section{BnTTS}

% \textbf{Preliminaries:} Given a text sequence with $N$ tokens, $\mathbf{T} = \{t_1, t_2, \dots, t_N\}$, and a speaker's mel-spectrogram $\mathbf{S} = \{s_1, s_2, \dots, s_L\}$, our objective is to generate speech $\hat{\mathbf{Y}}$ that matches the speaker's characteristics. Let $\mathbf{Y} = \{y_1, y_2, \dots, y_M\}$ denote the ground truth mel-spectrogram frames for the target speech. 

% The framework aims to synthesize $\hat{\mathbf{Y}}$ directly from $\mathbf{T}$ and $\mathbf{S}$, such that:
% \[
% \hat{\mathbf{Y}} = \mathcal{F}(\mathbf{T}, \mathbf{S})
% \]
% where $\mathcal{F}$ is the model responsible for producing speech conditioned on both the text and the speaker's spectrogram.

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=1.001\linewidth]{resources/hqtts.png} 
%     \caption{Overview of BnTTS Model} 
%     \label{fig:xtts_train_diagram}
% \end{figure}


% % \noindent \textbf{VQ-VAE:} Our method employs a Vector-Quantized Variational AutoEncoder (VQ-VAE) \cite{tortoise} as a speech tokenizer. The VQ-VAE transforms mel-spectrogram frames \(\mathbf{Y}\) into discrete codes \(\mathbf{z} \in \mathcal{C}\), where \(\mathcal{C}\) is the learned codebook of embeddings.

% \noindent \textbf{VQ-VAE:} Our method uses a Vector Quantized-Variational AutoEncoder (VQ-VAE) \cite{tortoise} to encode mel-spectrogram frames $\mathbf{Y}$ into discrete codes. The VQ-VAE effectively functions as speech tokenzier with a finite vocabulary.
% % latent vectors $\mathbf{Y_z} \in \mathbb{R}^{M \times d}$, where $d$ is the dimensionality of the model.

% \noindent \textbf{Conditioning Encoder \& Perceiver Resampler:}
% The Conditioning Encoder \cite{casanova2024xtts} consists of $l$ layers of $k$-head Scaled Dot-Product Attention, followed by a Perceiver Resampler. Each attention layer processes the input features to capture both local and global contexts.

% Given the speaker spectrogram $\mathbf{S}$, it is first transformed into an intermediate representation $\mathbf{S_z} \in \mathbb{R}^{L \times d}$. Each attention layer applies a scaled dot-product attention mechanism:
% \[
% \text{Attention}(\mathbf{Q}, \mathbf{K}, \mathbf{V}) = \text{softmax}\left(\frac{\mathbf{Q}\mathbf{K}^\top}{\sqrt{d}}\right) \mathbf{V}
% \]
% where $\mathbf{Q}$, $\mathbf{K}$, and $\mathbf{V}$ are projections of $\mathbf{S_z}$, computed over $k$ attention heads. The output from the final attention layer is passed through a Perceiver Resampler to produce a fixed output dimensionality.

% The Perceiver Resampler generates a fixed number of sequences $P$ from $L$. This resampling step ensures that the final output, $\mathbf{R} \in \mathbb{R}^{P \times d}$, has a fixed size $P$, independent of the variable input length $L$.


% \noindent \textbf{Text Encoder:} This step consists of a simple embedding layer that projects the input text tokens $\mathbf{T} = \{t_1, t_2, \dots, t_N\}$ into a continuous embedding space. The tokens are mapped to embeddings $\mathbf{T_e} \in \mathbb{R}^{N \times d}$, where $d$ is the embedding dimension.

% \noindent \textbf{LLM:}
% In this framework, we utilize the decoder portion of the transformer-based LLM \cite{radford2019language}. The  speaker embeddings $\mathbf{S_p}$, text embeddings $\mathbf{T_e}$, and ground truth spectrogram embeddings $\mathbf{Y_z}$ are concatenated to form the input during training. Let $\mathbf{X}$ denote this combined input:
% \[
% \mathbf{X} = \mathbf{S_p}  \oplus \mathbf{T_e} \oplus \mathbf{Y_z}
% \]
% where $\oplus$ represents concatenation, which results in $\mathbf{X} \in \mathbb{R}^{(N + P + M) \times d}$.

% The LLM processes $\mathbf{X}$ through its layers, producing an output from the final layer denoted by $\mathbf{H} =  \{ h_1^S, h_2^S, \dots, h_M^S, h_1^T, h_2^T, \dots, h_N^T, h_1^Y, h_2^Y, \dots, h_P^Y \}$, where $\mathbf{H} \in \mathbb{R}^{(N + P + M) \times d}$. Each component of $\mathbf{H}$ corresponds to the hidden states for the text, speaker, and spectrogram embeddings.

% During inference, only the text and speaker embeddings are concatenated, forming the input as:
% \[
% \mathbf{X} = \mathbf{S_p} \oplus \mathbf{T_e}
% \]
% The LLM then generates spectrogram embeddings $\{h_1^Y, h_2^Y, \dots, h_P^Y\}$, which serve as the predicted output speech representation.

% \noindent \textbf{HiFi-GAN Decoder: }
% The HiFi-GAN Decoder \cite{kong2020hifi} converts the LLM's output into realistic speech, preserving the speaker's unique characteristics. During training, it uses the ground truth spectrogram representation, whereas in inference, it uses the predicted spectrogram. Let $\mathbf{H}_\text{Y} = \{h_1^Y, h_2^Y, \dots, h_P^Y\} \in \mathbb{R}^{P \times d}$ represent spectrogram embedding.

% The speaker embedding $\mathbf{S}$ is resized to match $\mathbf{H}_\text{Y}$, resulting in $\mathbf{S}' \in \mathbb{R}^{P \times d}$. We then combine these by adding them element-wise and feeding them into the HiFi-GAN decoder, which produces the final audio waveform $\mathbf{W}$:
% \[
% \mathbf{W} = g_\text{HiFi}(\mathbf{H}_\text{Y} + \mathbf{S}')
% \]

% In this way, HiFi-GAN decoder generates speech that reflects the input text while maintaining the speaker’s unique sound qualities.

% \noindent \textbf{Training Objectives: } Our training process incorporates three different objectives. The first is the text generation objective, which helps the model predict future tokens based on the given text, improving its understanding of the sequence and aiding in advanced speech prediction. The second objective is audio generation, which aligns the synthesized audio with the input text. The third is the HiFi-GAN objective, which learns to transform the LLM's latents to speech signals via adversarial training. Details on each objective function can be found in Appendix C.


==> sections/Evaluation_Dataset.tex <==


\section{Evaluation Dataset}

For evaluating the performance of our TTS system, we curated two datasets: BnStudioEval and BnTTSTextEval, each serving distinct evaluation purposes.

\begin{itemize}
    \item \textbf{BnStudioEval}: This dataset comprises 100 high-quality instances (text and audio pair) taken from our in-house studio recordings. This dataset was selected to assess the model’s capability in replicating high-fidelity speech output with speaker impersonation. 
    
    \item \textbf{BnTTSTextEval}: The BnTTSTextEval dataset encompasses three subsets: \begin{itemize}
        \item \textbf{BengaliStimuli53}: A linguist-curated set of 53 instances, created to cover a comprehensive range of Bengali phonetic elements. This subset ensures that the model handles diverse phonemes.
        % Sample example: তোমাদের পড়াশুনা ধ্যানি ও গুরুমুখী নয়, বরং বাজারভিত্তিক।পূর্বসূরী অনেকের মত তোমরাও অনেকাংশে নিজের চিত্ত ও বোধকে গবেষণায় পূর্ণ করার চেয়ে ঘুষ খেয়ে ঘরে ফার্নিচারের মেলা বসাতে চাও, আর ঘৃত দিয়ে কিচেন।
        
        \item \textbf{BengaliNamedEntity1000}: A set of 1,000 instances focusing on proper nouns such as person, place, and organization names. This subset tests the model's handling of named entities, which is crucial for real-world conversational accuracy.
        % Sample Example: ময়মনসিংহ বিভাগের জেলাগুলো হচ্ছে শেরপুর, ময়মনসিংহ, জামালপুর, নেত্রকোণা।
        \item \textbf{ShortText200}: Composed of 200 instances, this subset includes short sentences  filler words, and common conversational phrases (less than three words) to evaluate the model’s performance in natural, day-to-day dialogue scenarios.
        % Sample Example: কি বলছেন?
    \end{itemize}  
\end{itemize}

The BnStudioEval dataset, with reference audio for each text, will be for reference-aware evaluation, while BnTTSTextEval supports reference-independent evaluation. Together, these datasets provide a comprehensive basis for evaluating various aspects of our TTS performance, including phonetic diversity, named entity pronunciation, and conversational fluency. 



==> sections/Speech_Generation.tex <==
\section{Speech Generation}
\subsection{Synthesizing Short Sequences}

The generation of short audio sequences presents challenges in the BnTTS model, particularly for texts containing fewer than 30 characters when using the default generation settings (Temperature \(T = 0.85\) and TopK = 50). The primary issues observed are twofold: (1) the generated speech often lacks intelligibility, and (2) the output speech tends to be longer than expected.

To investigate these challenges, we curated a subset of 23 short text-speech pairs from the BnStudioEval dataset. For evaluation, we utilize the Character Error Rate (CER) metric to assess intelligibility, and we introduce the Audio Duration Equality metric to evaluate the alignment between the generated and reference audio durations. The Audio Duration Equality Score quantifies the equality between two audio sample durations, \(a\) and \(b\), producing values between 0 and 1, where a score of 1 indicates identical durations. The metric is defined as:

\begin{equation}
    \text{DurationEquality}(a, b) = \frac{1}{\max\left(\frac{a}{b}, \frac{b}{a}\right)}
\end{equation}



This score approaches 1 as the durations of \(a\) and \(b\) become more equal, providing an effective measure of  discrepancy between duration of reference audio and synthesized audio .


\paragraph{Effect of Short Prompt}
Under the default settings (Exp. 1 in Table X), the model achieves a Character Error Rate (CER) of 0.081 and a Duration Equality Score of 0.699. We hypothesize that the model's inability to accurately synthesize short speech stems from its training process. During training, the model reserves between 1 to 6 seconds of audio for speaker prompting. For audio shorter than 1 second, the model uses half of the audio as the prompt. This implies that the model is accustomed to short audio prompts for short sequences. By aligning the inference process with this training strategy and using short prompts, the generation performance improves markedly, as evidenced by a higher Duration Equality Score of 0.820 and a lower CER of 0.029 in Exp. 2.

\paragraph{Effect of Temperature and Top-K Sampling}
The default temperature (\(T = 0.85\)) and top-K value (50) were found to be sub-optimal for generating short sequences. By adjusting the temperature to \(T = 1.0\) and reducing the top-K value to 2, we observed an improvement in the Duration Equality Score from 0.699 to 0.701, accompanied by a substantial reduction in CER, from 0.081 to 0.023 (as shown in Exp. 3).

\paragraph{Effect of Both Short Prompts and Temperature, Top-K}
Combining short prompts with the adjusted temperature and top-K values yielded the best results. In this configuration, the Duration Equality Score improved to 0.827, with a CER of 0.015, demonstrating that both factors are crucial for accurate short sequence generation.

The ablation study demonstrates that employing short prompts in combination with fine-tuning temperature and top-K values is essential for optimizing short sequence generation in the BnTTS model.

\begin{table}[H]
\centering

    \begin{tabular}{c|l}
        \hline
        \textbf{Variable} & \textbf{Description} \\ \hline
        \( \mathbf{T} \) & Text sequence with \( N \) tokens \\ \hline
        \( N \) & Number of tokens in the text sequence \\ \hline
        \( \mathbf{S} \) & Speaker's mel-spectrogram with \( L \) frames \\ \hline
        \( \hat{\mathbf{Y}} \) & Generated speech that matches the speaker's characteristics \\ \hline
        \( \mathbf{Y} \) & Ground truth mel-spectrogram frames for the target speech \\ \hline
        \( \mathcal{F} \) & Model responsible for producing speech conditioned on both the text and the speaker's spectrogram \\ \hline
        \( \mathbf{z} \) & Discrete codes transformed from mel-spectrogram frames using VQ-VAE \\ \hline
        \( \mathcal{C} \) & Codebook of discrete codes from VQ-VAE \\ \hline
        \( l \) & Number of layers in the Conditioning Encoder \\ \hline
        \( k \) & Number of attention heads in Scaled Dot-Product Attention \\ \hline
        \( \mathbf{S_z} \) & Intermediate representation of speaker spectrogram in \( \mathbb{R}^{L \times d} \) \\ \hline
        \( d \) & Dimensionality of each token or embedding \\ \hline
        \( \mathbf{Q}, \mathbf{K}, \mathbf{V} \) & Projections of \( \mathbf{S_z} \) used in scaled dot-product attention \\ \hline
        \( P \) & Fixed number of sequences produced by the Perceiver Resampler \\ \hline
        \( \mathbf{R} \) & Fixed-size output from the Perceiver Resampler in \( \mathbb{R}^{P \times d} \) \\ \hline
        \( \mathbf{T_e} \) & Continuous embedding space of text tokens in \( \mathbb{R}^{N \times d} \) \\ \hline
        \( \mathbf{S_p} \) & Speaker embeddings \\ \hline
        \( \mathbf{Y_z} \) & Ground truth spectrogram embeddings \\ \hline
        \( \mathbf{X} \) & Combined input during training: concatenation of speaker, text, and spectrogram embeddings \\ \hline
        \( \oplus \) & Concatenation operation \\ \hline
        \( \mathbf{H} \) & Output from the LLM consisting of hidden states for text, speaker, and spectrogram embeddings \\ \hline
        \( \mathbf{H}_\text{Y} \) & Spectrogram embedding from LLM output used for HiFi-GAN \\ \hline
        \( \mathbf{S}' \) & Resized speaker embedding to match \( \mathbf{H}_\text{Y} \) \\ \hline
        \( \mathbf{W} \) & Final audio waveform produced by HiFi-GAN \\ \hline
        \( g_\text{HiFi} \) & HiFi-GAN function converting spectrogram embeddings to audio waveform \\ \hline
    \end{tabular}
    \label{tab:variables_descriptions}
    \caption{Table of Variables and Descriptions}
\end{table}

% \section{Results and Discussion}

% To evaluate the performance of our Bengali TTS system, we employed a combination of subjective and objective metrics across two datasets: BnStudioEval and BnTTSTextEval. The BnStudioEval dataset, consisting of high-quality recordings, was used for reference-aware evaluation, while BnTTSTextEval encompassed subsets focusing on phonetic diversity, named entity pronunciation, and conversational fluency for reference-independent evaluation. The metrics used include subjective measures such as SMOS and objective measures like CER, UTMOS, SECS, and SpeechBERT Precision.



% \subsection{Reference-aware Evaluation (BnStudioEval)}
% Table 1 presents the comparative performance of various TTS systems evaluated on the BnStudioEval dataset. Among the synthetic methods, AzureTTS exhibited the best performance with the lowest Character Error Rate (CER) and the highest UTMOS score, outperforming all other synthetic methods, including Ground Truths (GT) in terms of transcription accuracy. However, interestingly, the CER of the GT remains lower than that of BnTTS synthesized outputs. As expected, the GT, serving as a reference standard, outperforms all synthetic systems across key subjective metrics such as SMOS (4.671), Naturalness (4.625), and Clarity (4.9). In this context, the proposed BnTTS system closely follows, achieving competitive scores in SMOS (4.584), Naturalness (4.531), and Clarity (4.898).

% Regarding speaker similarity, the GT achieved SECS scores of 1.0 when compared to reference audios and 0.361 when compared to the speaker prompt. BnTTS also performed well, with an SECS(Ref.) score of 0.513 and an SECS(Prompt) score of 0.335, falling short of the ground truth by only 0.031 in the latter metric. Additionally, BnTTS received a SpeechBERT Precision score of 0.796, compared to the perfect score of 1.0 set by the ground truth.

% It should be noted that IndicTTS, GTTS, and AzureTTS lack speaker impersonation capabilities, rendering them inapplicable for reference-aware metrics such as SECS and SpeechBERT Precision. Consequently, these metrics were not calculated for these systems.


% \subsection{Reference-independent Evaluation (BnTTSTextEval)}
% Table 2 presents the comparative performance of various TTS systems evaluated on the BnTTSTextEval dataset, encompassing three distinct subsets: BengaliStimuli53, BengaliNamedEntity1000, and ShortText200. The trend observed in the BnStudioEval dataset persists here as well. AzureTTS and GTTS consistently trade leading positions in transcription accuracy (CER) and automated quality prediction (UTMOS), with BnTTS following closely in third place, and IndicTTS trailing behind.

% BnTTS performs strongly in subjective evaluations, excelling in SMOS, Naturalness, and Intelligibility across the BengaliStimuli53 and BengaliNamedEntity1000 subsets. However, it falls slightly behind AzureTTS in the ShortText200 subset, which focuses on model performance in short texts. Despite this, BnTTS overall, remains the top-performing system in all subjective metrics, delivering the highest average scores in SMOS(4.383), Naturalness(4.313), and Clarity(4.737).


